Tempas: Temporal Archive Search Based on Tags

Limited search and access patterns over Web archives have been well documented. One of the key reasons is the lack of understanding of the user access patterns over such collections, which in turn is attributed to the lack of effective search interfaces. Current search interfaces for Web archives are (a) either purely navigational or (b) have sub-optimal search experience due to ineffective retrieval models or query modeling. We identify that external longitudinal resources, such as social bookmarking data, are crucial sources to identify important and popular websites in the past. To this extent we present Tempas, a tag-based temporal search engine for Web archives. Websites are posted at specific times of interest on several external platforms, such as bookmarking sites like Delicious. Attached tags not only act as relevant descriptors useful for retrieval, but also encode the time of relevance. With Tempas we tackle the challenge of temporally searching a Web archive by indexing tags and time. We allow temporal selections for search terms, rank documents based on their popularity and also provide meaningful query recommendations by exploiting tag-tag and tag-document co-occurrence statistics in arbitrary time windows. Finally, Tempas operates as a fairly non-invasive indexing framework. By not dealing with contents from the actual Web archive it constitutes an attractive and low-overhead approach for quick access into Web archives.

==> architecture.tex <==

\section{Retrieval}
\label{sec:retrieval}

Our retrieval model is based on three assumptions:
\begin{enumerate}
\item Most relevant websites in a given time frame with respect to certain query tags are also most frequently tagged with the query terms during this time frame.
\item More relevant versions of a website in a given time frame with respect to a set of query tags are tagged with more of these tags and less other tags.
\item Most frequently co-occurring tags of given query tags in a certain time frame represent their most related tags/topics during this time frame. 
\end{enumerate}

These three assumptions build different stages in the exploration and retrieval process of \textit{tempas}. Every exploration task starts with a query, which is a set of tags $T_\text{query}$. This may also be empty in case an exploration of the most prominent topics at a time is intended. In addition to the query, a time period $p_\text{query}$ is given. Based on these two inputs, \textit{tempas} retrieves tags as well as websites together with several versions of every website. These components are obtained from the delicious records in our dataset $D$. A record $r \in D$ constitutes a version $v_r$ of a particular website at a given time that has been tagged with a set of tags $T_r$: $r = (v_r, T_r)$. A subset of these records $D_{T, p} \subset D$ can be specified by a set of tags $T$ and a time period $p$. It includes only those records $r \in D$ that are tagged with all tag in $T$ ($T \cap T_r = T$) and represents a website's version within time period $p$ ($\text{start}(p) \leq \text{time}(v_r) \leq \text{end}(p)$.

For tag retrieval, all tags that co-occur with all query tags $T_\text{query}$ during $p_\text{query}$ are considered as relevant:
\[T_\text{rel} = \bigcap_{t \in T_\text{query}} \{T_r | r \in D_{\{t\},p_\text{query}}\}\]

Thus, tags are required to co-occur with all tags $t \in T_\text{query}$ during $p_\text{query}$, however, not necessarily in the same records.

Similarly for the retrieval of websites, those that are tagged with all query tags $T_\text{query}$ during $p_\text{query}$ are considered as relevant:
\[S_\text{rel} = \bigcap_{t \in T_\text{query}} \{\text{url}(v_r) | r \in D_{\{t\},p_\text{query}}\}\]

Both tags and websites are thus required to co-occur or to be tagged, respectively, with all tags $t \in T_\text{query}$ during $p_\text{query}$, however, not necessarily in the same records.

The third stage of the retrieval process is the retrieval of relevant versions of a website $s \in S_\text{rel}$ with respect to the query and time period under consideration. However, according to the statement above, even if a website was tagged with all query tags $T_\text{query}$ during the period $p_\text{query}$, it is possible that none of the records $r \in D$ include all query tags in $T_\text{query}$ in period $p_\text{query}$. Therefore, we consider all versions of the website in period $p_\text{query}$ relevant that are tagged with at least one the query tags. $V_\text{rel}$ is a subset of $D$, which besides the relevant versions also includes the tags a version has been tagged with:
\[V_\text{rel}(s) = \bigcup_{t \in T_\text{query}} \{r \in D_{\{t\},p_\text{query}} | url(r) = s \}\]

After retrieval, all three components undergo a ranking which weights their relevance in terms of the query tags and period.

\section{Ranking}
\label{sec:ranking}

The ranking is again based on the above stated assumptions (s. Sec.~\ref{sec:retrieval}). According to our first assumption, the more frequently a tag co-occurs with the query tags $T_\text{query}$ in period $p_\text{query}$, the more related is this tag to the query. Therefore, our ranking function $R_\text{tags}(\tau)$ computes for all relevant tags $\tau \in T_\text{rel}$ the number of records in which the tag co-occurs with one of the query tags in $T_\text{query}$ during period $p_\text{query}$:
\[R_\text{tags}(\tau) = \sum_{t \in T_\text{query}} |\{r \in D_{\{t\},p_\text{query}} | \tau \in T_r \}|\]

Websites are first ranked among themselves before their versions are ranked within each website. The ranking of the relevant websites $s \in S_\text{rel}$ is based on our second assumption: the more often a website is tagged with one of the query tags $T_\text{query}$ in period $p_\text{query}$, the more relevant is this website for the query. According, the corresponding ranking function $R_\text{sites}(s)$ computes for all relevant websites $s \in S_\text{rel}$ the number of records in which the website is tagged with one of the query tags in $T_\text{query}$ during period $p_\text{query}$:
\[R_\text{sites}(s) = \sum_{t \in T_\text{query}} |\{r \in D_{\{t\},p_\text{query}} | s = url(v_r) \}|\]

Based on our third assumption, we rank the versions of the relevant websites according to their overlap of tags they have been tagged with and the query tags $T_\text{query}$: the more of the query tags a version is tagged with, the more relevant is it with respect to the query. As a second factor we consider the total number of tags a version is tagged with: the more non query tags it is tagged with, the less relevant is it with respect to the query. Accordingly, the corresponding ranking function computes a tuple, that is ranked by the first component first (i.e., tag overlap) and by the second component afterwards (i.e., number of tags). $R_\text{versions}(v)$ is defined for each version $v \in V_\text{rel}(s)$ of the relevant websites $s \in S_\text{sites}$ as follows:
\[R_\text{versions}(v) = (|T_v \cap T_\text{query}|, -|T_v|)\]

\section{Architecture}
\label{sec:architecture}

% \begin{figure*}[t!]
% \centering
% \includegraphics[width=\textwidth]{screenshot.png}
% \caption{Screenshot of \textit{tempas}, showing a search for \textit{www}, \textit{technology} and \textit{science} between May 2007 and March 2011.}
% \label{fig:screenshot}
% \end{figure*}

The core of \textit{tempas} is a collection of indexes and mappings, which are tailored for retrieving the above described result sets (s. Sec.~\ref{sec:retrieval}). All of them are build to provide retrieval with a monthly granularity. We created indexes to retrieve tags as well as websites based on a query consisting of tags $T_\text{query}$ and a time period $p_\text{query}$ (i.e., \textit{TagTagMapping}, \textit{TagUrlMapping}). Furthermore, we created a year and monthly based index to retrieve tags without proving tags as input (i.e., \textit{YearTagMapping}, \textit{MonthTagMapping}) for exploratory search in a particular time frame without providing tags as input. Another index allows fetching all versions of a website that have been tagged during a given time period together with the tags (i.e., \textit{UrlTagMapping}). For saving space, two mappings assign ids to tags and websites, which are used exclusively in all other indexes and mappings (i.e., \textit{IdTagMapping}, \textit{IdUrlMapping}). Even though there is much room for improvement and optimization of temporal indexes \citep{anand_index_2012, anand_efficient_2010}, the rather simple mappings created on a Hadoop cluster already allow the desired functionality. The following listing gives an overview of the different mappings and what data they store:
\begin{itemize}
\item \textbf{IdTagMapping}\\
Maps consecutive ID numbers to tags in alphabetical order.

\item \textbf{IdUrlMapping}\\
Maps consecutive ID numbers to websites (its URLs) in alphabetical order.

\item \textbf{TagTagMapping}\\
Maps a tag in a certain month to a list of all co-occurring tags, together with the number of co-occurrences in that month.

\item \textbf{YearTagMapping}\\
Maps a year to a list of all tags used in that year, together with the number of occurrences for each tag.

\item \textbf{MonthTagMapping}\\
Maps a month to a list of all tags used in that year, together with the number of occurrences for each tag.

\item \textbf{TagUrlMapping}\\
Maps a tag in a certain month to a list of all websites that were tagged with this tag, together with the number of taggings (i.e., considered as different versions of the website).  

\item \textbf{UrlTagMapping}\\
Maps a website in a certain month to a list of all tags the website was tagged with, together with a set of timestamps for each tag, which represent the different versions when the tag was used.
\end{itemize}

All indexes are ordered by their keys (i.e., ID, year, month or pair of tag and year or website and year, respectively). The fetching of the indexes is realized by web services, which are invoked separately for tags and websites as well as a single fetch for the versions with tags of each websites. After fetching the data, all items (i.e., tags, websites or versions) are ordered according the ranking functions in Sec.~\ref{sec:ranking}.

The query with tags as well as the time period, consisting of start year and month as well as end year and month, can be entered and selected at the top of the page, using the search input and the three sliders as shown in Fig.~\ref{fig:screenshot}. In this example the query tag is '\textit{www}' and the search is performed between May 2007 and March 2011. After issuing the query, the most relevant tags are fetched as described in Sec.~\ref{sec:retrieval} using \textit{TagTagMapping}. During fetching, the tag IDs are resolved using the \textit{IdTagMapping} and ranked as described in Sec.~\ref{sec:ranking}. The top related tags are presented in the horizontal bar below the query input section at the top of the page. After selecting a tag in the first bar, here '\textit{technology}', a new bar is created which shows the tags for the query '\textit{www}' and '\textit{technology}' with respect to the selected time period. This continues for each selected tag. After selecting '\textit{science}' a new bar is created showing the most related tags for the query '\textit{www}', '\textit{technology}' and '\textit{science}', and so on. This allows a exploration of the most relevant subtopics of the original query and specifying the query step by step with respect to the chosen time period. Initially, before any query has been entered, all tags relevant for the selected time period are fetched, using the \textit{YearTagMapping} as well as \textit{MonthTagMapping}.

For every new query the result list on the left below the tags is refreshed and shows the most relevant websites with respect to the query tags and time period. Due to the time-consuming intersection and lookup operations, this is performed in two steps in order to keep the website response and provide first results as quick as possible. First, the websites are fetched and ranked as described in Sec.~\ref{sec:retrieval} and Sec.~\ref{sec:ranking}, using the \textit{TagUrlMapping}. Once this is done, for every website the relevant versions are fetched and ranked, starting with the first ranked website, using the \textit{UrlTagMapping}. During the second fetch the website URL as well as all related tags are resolved using the \textit{IdTagMapping} and \textit{IdUrlMapping}. Results are displayed once they are completely fetched and formatted like in prominent search engines, such as \textit{Google} or \textit{Bing}. However, while these typically show a page title and a snippet, which is not available in our dataset (s. Sec~\ref{sec:dataset}), we generate a title from the most frequently used tags of the websites with respect the selected time period, but independently from the query. Instead of a snippet we show different versions of the page, ranked with respect to the query. The top version, according to the ranking (s. Sec.~\ref{sec:ranking}), is shown as the date when it was tagged as well as all its tags right below the URL of the website. Less relevant versions are shown below just as dates, where the corresponding tags are displayed on hovering the links.

By clicking on the title of a result, the most relevant version of the website gets loaded in the right frame, next to the results. The same happens by clicking on the date or any other date, which loads the corresponding version. This is realized using the Wayback Machine of the Internet Archive\footnote{\url{http://archive.org/web}}. If the website at the exact time of the selected version is not available, the Wayback Machine automatically shows the version of the website that precedes this time.


==> dataset.tex <==

\section{Dataset}
\label{sec:dataset}

Our work on \textit{tempas} is based on the data of \textit{Delicious} from 2003 to 2011, collected by \cite{socialbm0311}. The dataset, called \textit{SocialBM0311}, has been published online and is freely available\footnote{\url{http://www.zubiaga.org/datasets/socialbm0311}}. According to the publisher, \textit{SocialBM0311} ``contains the complete bookmarking activity for almost 2 million users from the launch of the social bookmarking website in 2003 to the end of March 2011'' with 339,897,227 bookmarks, 118,520,382 unique URLs, 14,723,731 unique tags and 1,951,207 users. Its size is 11GB of compressed, tab-separated text data with each line in the following form:

\texttt{<url\_md5   user\_id   url   unix\_timestamp   tags>}

For our work we only consider the last three components, URL, timestamp and the list of tags. In the following we will refer to a URL as \textit{website} and every record in the dataset for one website is referred to as a \textit{version}, referring to the website at the time represented by the timestamp.


==> rel-work.tex <==
\section{Related Work}
